Finiteness of cominuscule quantum K-theory

The product of two Schubert classes in the quantum K-theory ring of a homogeneous space X = G/P is a formal power series with coefficients in the Grothendieck ring of algebraic vector bundles on X. We show that if X is cominuscule, then this power series has only finitely many non-zero terms. The proof is based on a geometric study of boundary Gromov-Witten varieties in the Kontsevich moduli space, consisting of stable maps to X that take the marked points to general Schubert varieties and whose domains are reducible curves of genus zero. We show that all such varieties have rational singularities, and that boundary Gromov-Witten varieties defined by two Schubert varieties are either empty or unirational. We also prove a relative Kleiman-Bertini theorem for rational singularities, which is of independent interest. A key result is that when X is cominuscule, all boundary Gromov-Witten varieties defined by three single points in X are rationally connected.

==> cayley.tex <==
\section{Quantum $K$-theory of the Cayley plane}\label{sec:cayley}

We use the following notation for the $K$-theoretic Schubert classes
of $X = E_6/P_6$.  If there is exactly one Schubert variety $\Omega
\subset X$ of codimension $d$, then we set $\cO_d = \cO_\Omega \in
K(X)$.  The Schubert classes that are not uniquely determined by their
codimension are named as follows.\smallskip

\noindent
$\cO_{4} = [\cO_{X(s_5s_4s_3s_1s_6s_5s_4s_2s_3s_4s_5s_6)}]$ ;  
$\cO'_{4} = [\cO_{X(s_2s_4s_3s_1s_6s_5s_4s_2s_3s_4s_5s_6)}]$ ;\\ 
$\cO_{5} = [\cO_{X(s_2s_4s_3s_1s_5s_4s_2s_3s_4s_5s_6)}]$ ;  
$\cO'_{5} = [\cO_{X(s_4s_3s_1s_6s_5s_4s_2s_3s_4s_5s_6)}]$ ;\\
$\cO_{6} = [\cO_{X(s_4s_3s_1s_5s_4s_2s_3s_4s_5s_6)}]$ ;  
$\cO'_{6} = [\cO_{X(s_3s_1s_6s_5s_4s_2s_3s_4s_5s_6)}]$ ;\\
$\cO_{7} = [\cO_{X(s_3s_1s_5s_4s_2s_3s_4s_5s_6)}]$ ;  
$\cO'_{7} = [\cO_{X(s_1s_6s_5s_4s_2s_3s_4s_5s_6)}]$ ;\\
$\cO_{8} = [\cO_{X(s_3s_1s_4s_2s_3s_4s_5s_6)}]$;  
$\cO'_{8} = [\cO_{X(s_1s_5s_4s_2s_3s_4s_5s_6)}]$;  
$\cO''_{8} = [\cO_{X(s_6s_5s_4s_2s_3s_4s_5s_6)}]$;\\
$\cO_{9} = [\cO_{X(s_1s_4s_2s_3s_4s_5s_6)}]$ ;  
$\cO'_{9} = [\cO_{X(s_5s_4s_2s_3s_4s_5s_6)}]$ ; 
$\cO_{10} = [\cO_{X(s_1s_2s_3s_4s_5s_6)}]$ ;\\
$\cO'_{10} = [\cO_{X(s_4s_2s_3s_4s_5s_6)}]$ ; 
$\cO_{11} = [\cO_{X(s_1s_3s_4s_5s_6)}]$ ; 
$\cO'_{11} = [\cO_{X(s_2s_3s_4s_5s_6)}]$ ;\\
$\cO_{12} = [\cO_{X(s_2s_4s_5s_6)}]$ ;  
$\cO'_{12} = [\cO_{X(s_3s_4s_5s_6)}]$.
\medskip

With this notation, the multiplication table for $\QK(X)$ is given
below.  The products are computed based on
\cite[Thm.~7.2]{buch.mihalcea:quantum} and
\cite[Thm.~3.5]{chaput.perrin:rationality}.\smallskip

\noindent
{\SMALL
$\cO_{1} \star \cO_{1} = \cO_{2}$ ; 
$\cO_{2} \star \cO_{1} = \cO_{3}$ ; 
$\cO_{2} \star \cO_{2} = \cO_{4} + \cO'_{4} - \cO'_{5}$ ; 
$\cO_{3} \star \cO_{1} = \cO_{4} + \cO'_{4} - \cO'_{5}$ ;\\
$\cO_{3} \star \cO_{2} = \cO_{5} + 2\cO'_{5} - 2\cO_{6} - \cO'_{6} + \cO_{7}$ ; 
$\cO_{3} \star \cO_{3} = 3\cO_{6} + 2\cO'_{6} - 5\cO_{7} - \cO'_{7} + \cO_{8} + 2\cO'_{8} - \cO_{9}$ ;\\
$\cO_{4} \star \cO_{1} = \cO'_{5}$ ;
$\cO_{4} \star \cO_{2} = \cO_{6} + \cO'_{6} - \cO_{7}$ ;
$\cO_{4} \star \cO_{3} = 2\cO_{7} + \cO'_{7} - \cO_{8} - 2\cO'_{8} + \cO_{9}$ ;\\
$\cO_{4} \star \cO_{4} = \cO_{8} + \cO'_{8} + \cO''_{8} - \cO_{9} - \cO'_{9}$ ;
$\cO'_{4} \star \cO_{1} = \cO_{5} + \cO'_{5} - \cO_{6}$ ;
$\cO'_{4} \star \cO_{2} = 2\cO_{6} + \cO'_{6} - 2\cO_{7}$ ;\\
$\cO'_{4} \star \cO_{3} = 3\cO_{7} + \cO'_{7} - 2\cO_{8} - 3\cO'_{8} + 2\cO_{9}$ ;
$\cO'_{4} \star \cO_{4} = \cO_{8} + 2\cO'_{8} - 2\cO_{9}$ ;\\
$\cO'_{4} \star \cO'_{4} = 2\cO_{8} + 2\cO'_{8} + \cO''_{8} - 3\cO_{9} - 2\cO'_{9} + \cO'_{10}$ ;
$\cO_{5} \star \cO_{1} = \cO_{6}$ ;\\
$\cO_{5} \star \cO_{2} = \cO_{7}$ ;
$\cO_{5} \star \cO_{3} = \cO_{8} + \cO'_{8} - \cO_{9}$ ;
$\cO_{5} \star \cO_{4} = \cO_{9}$ ;
$\cO_{5} \star \cO'_{4} = \cO_{9} + \cO'_{9} - \cO'_{10}$ ;
$\cO_{5} \star \cO_{5} = \cO'_{10}$ ;\\
$\cO'_{5} \star \cO_{1} = \cO_{6} + \cO'_{6} - \cO_{7}$ ;
$\cO'_{5} \star \cO_{2} = 2\cO_{7} + \cO'_{7} - \cO_{8} - 2\cO'_{8} + \cO_{9}$ ;\\
$\cO'_{5} \star \cO_{3} = 2\cO_{8} + 3\cO'_{8} + \cO''_{8} - 5\cO_{9} - 3\cO'_{9} + \cO_{10} + 3\cO'_{10} - \cO'_{11}$ ;\\
$\cO'_{5} \star \cO_{4} = 2\cO_{9} + 2\cO'_{9} - \cO_{10} - 3\cO'_{10} + \cO'_{11}$ ;
$\cO'_{5} \star \cO'_{4} = 3\cO_{9} + 2\cO'_{9} - 2\cO_{10} - 4\cO'_{10} + 2\cO'_{11}$ ;\\
$\cO'_{5} \star \cO_{5} = \cO_{10} + \cO'_{10} - \cO'_{11}$ ;
$\cO'_{5} \star \cO'_{5} = 2\cO_{10} + 4\cO'_{10} - \cO_{11} - 6\cO'_{11} + \cO_{12} + 2\cO'_{12} - \cO_{13}$ ;\\
$\cO_{6} \star \cO_{1} = \cO_{7}$ ;
$\cO_{6} \star \cO_{2} = \cO_{8} + \cO'_{8} - \cO_{9}$ ;
$\cO_{6} \star \cO_{3} = 2\cO_{9} + \cO'_{9} - \cO_{10} - 2\cO'_{10} + \cO'_{11}$ ;\\
$\cO_{6} \star \cO_{4} = \cO_{10} + \cO'_{10} - \cO'_{11}$ ;
$\cO_{6} \star \cO'_{4} = \cO_{10} + 2\cO'_{10} - 2\cO'_{11}$ ;
$\cO_{6} \star \cO_{5} = \cO'_{11}$ ;\\
$\cO_{6} \star \cO'_{5} = \cO_{11} + 2\cO'_{11} - \cO_{12} - 2\cO'_{12} + \cO_{13}$ ;
$\cO_{6} \star \cO_{6} = \cO_{12} + \cO'_{12} - \cO_{13}$ ;
$\cO'_{6} \star \cO_{1} = \cO_{7} + \cO'_{7} - \cO'_{8}$ ;\\
$\cO'_{6} \star \cO_{2} = \cO_{8} + 2\cO'_{8} + \cO''_{8} - 2\cO_{9} - 2\cO'_{9} + \cO'_{10}$ ;
$\cO'_{6} \star \cO_{3} = 3\cO_{9} + 3\cO'_{9} - 2\cO_{10} - 6\cO'_{10} + 3\cO'_{11}$ ;\\
$\cO'_{6} \star \cO_{4} = \cO_{10} + 3\cO'_{10} - 3\cO'_{11}$ ;
$\cO'_{6} \star \cO'_{4} = 2\cO_{10} + 3\cO'_{10} - \cO_{11} - 4\cO'_{11} + \cO'_{12}$ ;\\
$\cO'_{6} \star \cO_{5} = \cO_{11} + \cO'_{11} - \cO'_{12}$ ;
$\cO'_{6} \star \cO'_{5} = \cO_{11} + 4\cO'_{11} - 3\cO_{12} - 4\cO'_{12} + 3\cO_{13}$ ;\\
$\cO'_{6} \star \cO_{6} = \cO_{12} + 2\cO'_{12} + q - 2\cO_{13} - 2q\cO_{1} + q\cO_{2}$ ;
$\cO'_{6} \star \cO'_{6} = 3\cO_{12} + 3\cO'_{12} - 6\cO_{13} + \cO_{14}$ ;\\
$\cO_{7} \star \cO_{1} = \cO_{8} + \cO'_{8} - \cO_{9}$ ;
$\cO_{7} \star \cO_{2} = 2\cO_{9} + \cO'_{9} - \cO_{10} - 2\cO'_{10} + \cO'_{11}$ ;\\
$\cO_{7} \star \cO_{3} = 2\cO_{10} + 3\cO'_{10} - \cO_{11} - 5\cO'_{11} + \cO_{12} + 2\cO'_{12} - \cO_{13}$ ;\\
$\cO_{7} \star \cO_{4} = \cO_{11} + 2\cO'_{11} - \cO_{12} - 2\cO'_{12} + \cO_{13}$ ;
$\cO_{7} \star \cO'_{4} = \cO_{11} + 3\cO'_{11} - 2\cO_{12} - 3\cO'_{12} + 2\cO_{13}$ ;\\
$\cO_{7} \star \cO_{5} = \cO_{12} + \cO'_{12} - \cO_{13}$ ;
$\cO_{7} \star \cO'_{5} = 2\cO_{12} + 3\cO'_{12} + q - 5\cO_{13} - 3q\cO_{1} + \cO_{14} + 3q\cO_{2} - q\cO_{3}$ ;\\
$\cO_{7} \star \cO_{6} = 2\cO_{13} + q\cO_{1} - \cO_{14} - 2q\cO_{2} + q\cO_{3}$ ;
$\cO_{7} \star \cO'_{6} = 3\cO_{13} + 3q\cO_{1} - 2\cO_{14} - 6q\cO_{2} + 3q\cO_{3}$ ;\\
$\cO_{7} \star \cO_{7} = 2\cO_{14} + 3q\cO_{2} - \cO_{15} - 5q\cO_{3} + q\cO_{4} + 2q\cO'_{4} - q\cO'_{5}$ ;
$\cO'_{7} \star \cO_{1} = \cO'_{8} + \cO''_{8} - \cO'_{9}$ ;\\
$\cO'_{7} \star \cO_{2} = \cO_{9} + 2\cO'_{9} - 2\cO'_{10}$ ;
$\cO'_{7} \star \cO_{3} = \cO_{10} + 3\cO'_{10} - 3\cO'_{11}$ ;
$\cO'_{7} \star \cO_{4} = 2\cO'_{11} - \cO_{12}$ ;\\
$\cO'_{7} \star \cO'_{4} = \cO_{11} + 2\cO'_{11} - 2\cO'_{12}$ ;
$\cO'_{7} \star \cO_{5} = \cO'_{12} + q - q\cO_{1}$ ;
$\cO'_{7} \star \cO'_{5} = 2\cO_{12} + 2\cO'_{12} - 3\cO_{13}$ ;\\
$\cO'_{7} \star \cO_{6} = \cO_{13} + 2q\cO_{1} - 2q\cO_{2}$ ;
$\cO'_{7} \star \cO'_{6} = 3\cO_{13} - 2\cO_{14}$ ;
$\cO'_{7} \star \cO_{7} = \cO_{14} + 3q\cO_{2} - 3q\cO_{3}$ ;\\
$\cO'_{7} \star \cO'_{7} = 2\cO_{14} - \cO_{15}$ ;
$\cO_{8} \star \cO_{1} = \cO_{9}$ ;
$\cO_{8} \star \cO_{2} = \cO_{10} + \cO'_{10} - \cO'_{11}$ ;\\
$\cO_{8} \star \cO_{3} = \cO_{11} + 2\cO'_{11} - \cO_{12} - 2\cO'_{12} + \cO_{13}$ ;
$\cO_{8} \star \cO_{4} = \cO_{12} + \cO'_{12} + q - \cO_{13} - q\cO_{1}$ ;\\
$\cO_{8} \star \cO'_{4} = \cO_{12} + 2\cO'_{12} - 2\cO_{13}$ ;
$\cO_{8} \star \cO_{5} = \cO_{13}$ ;
$\cO_{8} \star \cO'_{5} = 2\cO_{13} + 2q\cO_{1} - \cO_{14} - 3q\cO_{2} + q\cO_{3}$ ;\\
$\cO_{8} \star \cO_{6} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;
$\cO_{8} \star \cO'_{6} = \cO_{14} + 3q\cO_{2} - 3q\cO_{3}$ ;\\
$\cO_{8} \star \cO_{7} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$ ;
$\cO_{8} \star \cO'_{7} = 2q\cO_{3} - q\cO_{4}$ ;\\
$\cO_{8} \star \cO_{8} = \cO_{16} + q\cO_{4} + q\cO'_{4} - q\cO_{5} - q\cO'_{5}$ ;
$\cO'_{8} \star \cO_{1} = \cO_{9} + \cO'_{9} - \cO'_{10}$ ;
$\cO'_{8} \star \cO_{2} = \cO_{10} + 2\cO'_{10} - 2\cO'_{11}$ ;\\
$\cO'_{8} \star \cO_{3} = \cO_{11} + 3\cO'_{11} - 2\cO_{12} - 3\cO'_{12} + 2\cO_{13}$ ;
$\cO'_{8} \star \cO_{4} = \cO_{12} + 2\cO'_{12} - 2\cO_{13}$ ;\\
$\cO'_{8} \star \cO'_{4} = 2\cO_{12} + 2\cO'_{12} + q - 3\cO_{13} - 2q\cO_{1} + q\cO_{2}$ ;
$\cO'_{8} \star \cO_{5} = \cO_{13} + q\cO_{1} - q\cO_{2}$ ;\\
$\cO'_{8} \star \cO'_{5} = 3\cO_{13} + 2q\cO_{1} - 2\cO_{14} - 4q\cO_{2} + 2q\cO_{3}$ ;
$\cO'_{8} \star \cO_{6} = \cO_{14} + 2q\cO_{2} - 2q\cO_{3}$ ;\\
$\cO'_{8} \star \cO'_{6} = 2\cO_{14} + 3q\cO_{2} - \cO_{15} - 4q\cO_{3} + q\cO'_{4}$ ;
$\cO'_{8} \star \cO_{7} = \cO_{15} + 3q\cO_{3} - 2q\cO_{4} - 3q\cO'_{4} + 2q\cO'_{5}$ ;\\
$\cO'_{8} \star \cO'_{7} = \cO_{15} + 2q\cO_{3} - 2q\cO'_{4}$ ;
$\cO'_{8} \star \cO_{8} = q\cO_{4} + 2q\cO'_{4} - 2q\cO'_{5}$ ;\\
$\cO'_{8} \star \cO'_{8} = \cO_{16} + 2q\cO_{4} + 2q\cO'_{4} - 2q\cO_{5} - 3q\cO'_{5} + q\cO_{6}$ ;
$\cO''_{8} \star \cO_{1} = \cO'_{9}$ ;
$\cO''_{8} \star \cO_{2} = \cO'_{10}$ ;
$\cO''_{8} \star \cO_{3} = \cO'_{11}$ ;\\
$\cO''_{8} \star \cO_{4} = \cO_{12}$ ;
$\cO''_{8} \star \cO'_{4} = \cO'_{12}$ ;
$\cO''_{8} \star \cO_{5} = q\cO_{1}$ ;
$\cO''_{8} \star \cO'_{5} = \cO_{13}$ ;
$\cO''_{8} \star \cO_{6} = q\cO_{2}$ ;
$\cO''_{8} \star \cO'_{6} = \cO_{14}$ ;\\
$\cO''_{8} \star \cO_{7} = q\cO_{3}$ ;
$\cO''_{8} \star \cO'_{7} = \cO_{15}$ ;
$\cO''_{8} \star \cO_{8} = q\cO_{4}$ ;
$\cO''_{8} \star \cO'_{8} = q\cO'_{4}$ ;
$\cO''_{8} \star \cO''_{8} = \cO_{16}$ ;\\
$\cO_{9} \star \cO_{1} = \cO_{10} + \cO'_{10} - \cO'_{11}$ ;
$\cO_{9} \star \cO_{2} = \cO_{11} + 2\cO'_{11} - \cO_{12} - 2\cO'_{12} + \cO_{13}$ ;\\
$\cO_{9} \star \cO_{3} = 2\cO_{12} + 3\cO'_{12} + q - 5\cO_{13} - 3q\cO_{1} + \cO_{14} + 3q\cO_{2} - q\cO_{3}$ ;
$\cO_{9} \star \cO_{4} = 2\cO_{13} + 2q\cO_{1} - \cO_{14} - 3q\cO_{2} + q\cO_{3}$;\\
$\cO_{9} \star \cO'_{4} = 3\cO_{13} + 2q\cO_{1} - 2\cO_{14} - 4q\cO_{2} + 2q\cO_{3}$ ;
$\cO_{9} \star \cO_{5} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;\\
$\cO_{9} \star \cO'_{5} = 2\cO_{14} + 4q\cO_{2} - \cO_{15} - 6q\cO_{3} + q\cO_{4} + 2q\cO'_{4} - q\cO'_{5}$ ;\\
$\cO_{9} \star \cO_{6} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$ ;
$\cO_{9} \star \cO'_{6} = \cO_{15} + 4q\cO_{3} - 3q\cO_{4} - 4q\cO'_{4} + 3q\cO'_{5}$ ;\\
$\cO_{9} \star \cO_{7} = \cO_{16} + 2q\cO_{4} + 3q\cO'_{4} - 3q\cO_{5} - 5q\cO'_{5} + 3q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;
$\cO_{9} \star \cO'_{7} = 2q\cO_{4} + 2q\cO'_{4} - 3q\cO'_{5}$ ;\\
$\cO_{9} \star \cO_{8} = 2q\cO_{5} + 2q\cO'_{5} - 3q\cO_{6} - q\cO'_{6} + q\cO_{7}$ ;
$\cO_{9} \star \cO'_{8} = 2q\cO_{5} + 3q\cO'_{5} - 4q\cO_{6} - 2q\cO'_{6} + 2q\cO_{7}$ ;\\
$\cO_{9} \star \cO''_{8} = q\cO'_{5}$ ;
$\cO_{9} \star \cO_{9} = 4q\cO_{6} + 2q\cO'_{6} - 6q\cO_{7} - q\cO'_{7} + q\cO_{8} + 2q\cO'_{8} - q\cO_{9}$ ;
$\cO'_{9} \star \cO_{1} = \cO'_{10}$ ;\\
$\cO'_{9} \star \cO_{2} = \cO'_{11}$ ;
$\cO'_{9} \star \cO_{3} = \cO_{12} + \cO'_{12} - \cO_{13}$ ;
$\cO'_{9} \star \cO_{4} = \cO_{13}$ ;
$\cO'_{9} \star \cO'_{4} = \cO_{13} + q\cO_{1} - q\cO_{2}$ ;\\
$\cO'_{9} \star \cO_{5} = q\cO_{2}$ ;
$\cO'_{9} \star \cO'_{5} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;
$\cO'_{9} \star \cO_{6} = q\cO_{3}$ ;
$\cO'_{9} \star \cO'_{6} = \cO_{15} + q\cO_{3} - q\cO'_{4}$ ;\\
$\cO'_{9} \star \cO_{7} = q\cO_{4} + q\cO'_{4} - q\cO'_{5}$ ;
$\cO'_{9} \star \cO'_{7} = \cO_{16} + q\cO'_{4} - q\cO_{5}$ ;
$\cO'_{9} \star \cO_{8} = q\cO'_{5}$ ;\\
$\cO'_{9} \star \cO'_{8} = q\cO_{5} + q\cO'_{5} - q\cO_{6}$ ;
$\cO'_{9} \star \cO''_{8} = q\cO_{5}$ ;
$\cO'_{9} \star \cO_{9} = q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;
$\cO'_{9} \star \cO'_{9} = q\cO_{6}$ ;\\
$\cO_{10} \star \cO_{1} = \cO_{11} + \cO'_{11} - \cO'_{12}$ ;
$\cO_{10} \star \cO_{2} = \cO_{12} + 2\cO'_{12} + q - 2\cO_{13} - 2q\cO_{1} + q\cO_{2}$ ;\\
$\cO_{10} \star \cO_{3} = 3\cO_{13} + 3q\cO_{1} - 2\cO_{14} - 6q\cO_{2} + 3q\cO_{3}$ ;
$\cO_{10} \star \cO_{4} = \cO_{14} + 3q\cO_{2} - 3q\cO_{3}$ ;\\
$\cO_{10} \star \cO'_{4} = 2\cO_{14} + 3q\cO_{2} - \cO_{15} - 4q\cO_{3} + q\cO'_{4}$ ;
$\cO_{10} \star \cO_{5} = \cO_{15} + q\cO_{3} - q\cO'_{4}$ ;\\
$\cO_{10} \star \cO'_{5} = \cO_{15} + 4q\cO_{3} - 3q\cO_{4} - 4q\cO'_{4} + 3q\cO'_{5}$ ;
$\cO_{10} \star \cO_{6} = \cO_{16} + q\cO_{4} + 2q\cO'_{4} - 2q\cO_{5} - 2q\cO'_{5} + q\cO_{6}$ ;\\
$\cO_{10} \star \cO'_{6} = 3q\cO_{4} + 3q\cO'_{4} - 6q\cO'_{5} + q\cO'_{6}$ ;
$\cO_{10} \star \cO_{7} = 3q\cO_{5} + 3q\cO'_{5} - 6q\cO_{6} - 2q\cO'_{6} + 3q\cO_{7}$ ;\\
$\cO_{10} \star \cO'_{7} = 3q\cO'_{5} - 2q\cO'_{6}$ ;
$\cO_{10} \star \cO_{8} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$ ;\\
$\cO_{10} \star \cO'_{8} = 3q\cO_{6} + 2q\cO'_{6} - 4q\cO_{7} - q\cO'_{7} + q\cO'_{8}$ ;
$\cO_{10} \star \cO''_{8} = q\cO'_{6}$ ;\\
$\cO_{10} \star \cO_{9} = 4q\cO_{7} + q\cO'_{7} - 3q\cO_{8} - 4q\cO'_{8} + 3q\cO_{9}$ ;
$\cO_{10} \star \cO'_{9} = q\cO_{7} + q\cO'_{7} - q\cO'_{8}$ ;\\
$\cO_{10} \star \cO_{10} = 3q\cO_{8} + 3q\cO'_{8} - 6q\cO_{9} + q\cO_{10}$ ;
$\cO'_{10} \star \cO_{1} = \cO'_{11}$ ;
$\cO'_{10} \star \cO_{2} = \cO_{12} + \cO'_{12} - \cO_{13}$ ;\\
$\cO'_{10} \star \cO_{3} = 2\cO_{13} + q\cO_{1} - \cO_{14} - 2q\cO_{2} + q\cO_{3}$ ;
$\cO'_{10} \star \cO_{4} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;\\
$\cO'_{10} \star \cO'_{4} = \cO_{14} + 2q\cO_{2} - 2q\cO_{3}$ ;
$\cO'_{10} \star \cO_{5} = q\cO_{3}$ ;
$\cO'_{10} \star \cO'_{5} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$ ;\\
$\cO'_{10} \star \cO_{6} = q\cO_{4} + q\cO'_{4} - q\cO'_{5}$ ;
$\cO'_{10} \star \cO'_{6} = \cO_{16} + q\cO_{4} + 2q\cO'_{4} - 2q\cO_{5} - 2q\cO'_{5} + q\cO_{6}$ ;\\
$\cO'_{10} \star \cO_{7} = q\cO_{5} + 2q\cO'_{5} - 2q\cO_{6} - q\cO'_{6} + q\cO_{7}$ ;
$\cO'_{10} \star \cO'_{7} = 2q\cO_{5} + q\cO'_{5} - 2q\cO_{6}$ ;\\
$\cO'_{10} \star \cO_{8} = q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;
$\cO'_{10} \star \cO'_{8} = 2q\cO_{6} + q\cO'_{6} - 2q\cO_{7}$ ;
$\cO'_{10} \star \cO''_{8} = q\cO_{6}$ ;\\
$\cO'_{10} \star \cO_{9} = 2q\cO_{7} + q\cO'_{7} - q\cO_{8} - 2q\cO'_{8} + q\cO_{9}$ ;
$\cO'_{10} \star \cO'_{9} = q\cO_{7}$ ;\\
$\cO'_{10} \star \cO_{10} = q\cO_{8} + 2q\cO'_{8} + q\cO''_{8} - 2q\cO_{9} - 2q\cO'_{9} + q\cO'_{10}$ ;
$\cO'_{10} \star \cO'_{10} = q\cO_{8} + q\cO'_{8} - q\cO_{9}$ ;\\
$\cO_{11} \star \cO_{1} = \cO'_{12} + q - q\cO_{1}$ ;
$\cO_{11} \star \cO_{2} = \cO_{13} + 2q\cO_{1} - 2q\cO_{2}$ ;
$\cO_{11} \star \cO_{3} = \cO_{14} + 3q\cO_{2} - 3q\cO_{3}$ ;\\
$\cO_{11} \star \cO_{4} = 2q\cO_{3} - q\cO_{4}$ ;
$\cO_{11} \star \cO'_{4} = \cO_{15} + 2q\cO_{3} - 2q\cO'_{4}$ ;
$\cO_{11} \star \cO_{5} = \cO_{16} + q\cO'_{4} - q\cO_{5}$ ;\\
$\cO_{11} \star \cO'_{5} = 2q\cO_{4} + 2q\cO'_{4} - 3q\cO'_{5}$ ;
$\cO_{11} \star \cO_{6} = 2q\cO_{5} + q\cO'_{5} - 2q\cO_{6}$ ;
$\cO_{11} \star \cO'_{6} = 3q\cO'_{5} - 2q\cO'_{6}$ ;\\
$\cO_{11} \star \cO_{7} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$ ;
$\cO_{11} \star \cO'_{7} = 2q\cO'_{6} - q\cO'_{7}$ ;
$\cO_{11} \star \cO_{8} = 2q\cO_{7} - q\cO_{8}$ ;\\
$\cO_{11} \star \cO'_{8} = 2q\cO_{7} + q\cO'_{7} - 2q\cO'_{8}$ ;
$\cO_{11} \star \cO''_{8} = q\cO'_{7}$ ;
$\cO_{11} \star \cO_{9} = 2q\cO_{8} + 2q\cO'_{8} - 3q\cO_{9}$ ;\\
$\cO_{11} \star \cO'_{9} = q\cO'_{8} + q\cO''_{8} - q\cO'_{9}$ ;
$\cO_{11} \star \cO_{10} = 3q\cO_{9} - 2q\cO_{10}$ ;
$\cO_{11} \star \cO'_{10} = q\cO_{9} + 2q\cO'_{9} - 2q\cO'_{10}$ ;\\
$\cO_{11} \star \cO_{11} = 2q\cO_{10} - q\cO_{11}$ ;
$\cO'_{11} \star \cO_{1} = \cO_{12} + \cO'_{12} - \cO_{13}$ ;
$\cO'_{11} \star \cO_{2} = 2\cO_{13} + q\cO_{1} - \cO_{14} - 2q\cO_{2} + q\cO_{3}$;\\
$\cO'_{11} \star \cO_{3} = 2\cO_{14} + 3q\cO_{2} - \cO_{15} - 5q\cO_{3} + q\cO_{4} + 2q\cO'_{4} - q\cO'_{5}$ ;
$\cO'_{11} \star \cO_{4} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$;\\
$\cO'_{11} \star \cO'_{4} = \cO_{15} + 3q\cO_{3} - 2q\cO_{4} - 3q\cO'_{4} + 2q\cO'_{5}$ ;
$\cO'_{11} \star \cO_{5} = q\cO_{4} + q\cO'_{4} - q\cO'_{5}$ ;\\
$\cO'_{11} \star \cO'_{5} = \cO_{16} + 2q\cO_{4} + 3q\cO'_{4} - 3q\cO_{5} - 5q\cO'_{5} + 3q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;\\
$\cO'_{11} \star \cO_{6} = q\cO_{5} + 2q\cO'_{5} - 2q\cO_{6} - q\cO'_{6} + q\cO_{7}$ ;
$\cO'_{11} \star \cO'_{6} = 3q\cO_{5} + 3q\cO'_{5} - 6q\cO_{6} - 2q\cO'_{6} + 3q\cO_{7}$ ;\\
$\cO'_{11} \star \cO_{7} = 3q\cO_{6} + 2q\cO'_{6} - 5q\cO_{7} - q\cO'_{7} + q\cO_{8} + 2q\cO'_{8} - q\cO_{9}$ ;
$\cO'_{11} \star \cO'_{7} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$ ;\\
$\cO'_{11} \star \cO_{8} = 2q\cO_{7} + q\cO'_{7} - q\cO_{8} - 2q\cO'_{8} + q\cO_{9}$ ;
$\cO'_{11} \star \cO'_{8} = 3q\cO_{7} + q\cO'_{7} - 2q\cO_{8} - 3q\cO'_{8} + 2q\cO_{9}$ ;\\
$\cO'_{11} \star \cO''_{8} = q\cO_{7}$ ;
$\cO'_{11} \star \cO_{9} = 2q\cO_{8} + 3q\cO'_{8} + q\cO''_{8} - 5q\cO_{9} - 3q\cO'_{9} + q\cO_{10} + 3q\cO'_{10} - q\cO'_{11}$ ;\\
$\cO'_{11} \star \cO'_{9} = q\cO_{8} + q\cO'_{8} - q\cO_{9}$ ;
$\cO'_{11} \star \cO_{10} = 3q\cO_{9} + 3q\cO'_{9} - 2q\cO_{10} - 6q\cO'_{10} + 3q\cO'_{11}$ ;\\
$\cO'_{11} \star \cO'_{10} = 2q\cO_{9} + q\cO'_{9} - q\cO_{10} - 2q\cO'_{10} + q\cO'_{11}$ ;
$\cO'_{11} \star \cO_{11} = q\cO_{10} + 3q\cO'_{10} - 3q\cO'_{11}$ ;\\
$\cO'_{11} \star \cO'_{11} = 2q\cO_{10} + 3q\cO'_{10} - q\cO_{11} - 5q\cO'_{11} + q\cO_{12} + 2q\cO'_{12} - q\cO_{13}$ ;
$\cO_{12} \star \cO_{1} = \cO_{13}$ ;\\
$\cO_{12} \star \cO_{2} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;
$\cO_{12} \star \cO_{3} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$ ;\\
$\cO_{12} \star \cO_{4} = \cO_{16} + q\cO_{4} + q\cO'_{4} - q\cO_{5} - q\cO'_{5}$ ;
$\cO_{12} \star \cO'_{4} = q\cO_{4} + 2q\cO'_{4} - 2q\cO'_{5}$ ;
$\cO_{12} \star \cO_{5} = q\cO'_{5}$ ;\\
$\cO_{12} \star \cO'_{5} = 2q\cO_{5} + 2q\cO'_{5} - 3q\cO_{6} - q\cO'_{6} + q\cO_{7}$ ;
$\cO_{12} \star \cO_{6} = q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;
$\cO_{12} \star \cO'_{6} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$;\\
$\cO_{12} \star \cO_{7} = 2q\cO_{7} + q\cO'_{7} - q\cO_{8} - 2q\cO'_{8} + q\cO_{9}$ ;
$\cO_{12} \star \cO'_{7} = 2q\cO_{7} - q\cO_{8}$ ;\\
$\cO_{12} \star \cO_{8} = q\cO_{8} + q\cO'_{8} + q\cO''_{8} - q\cO_{9} - q\cO'_{9}$ ;
$\cO_{12} \star \cO'_{8} = q\cO_{8} + 2q\cO'_{8} - 2q\cO_{9}$ ;
$\cO_{12} \star \cO''_{8} = q\cO_{8}$ ;\\
$\cO_{12} \star \cO_{9} = 2q\cO_{9} + 2q\cO'_{9} - q\cO_{10} - 3q\cO'_{10} + q\cO'_{11}$ ;
$\cO_{12} \star \cO'_{9} = q\cO_{9}$ ;
$\cO_{12} \star \cO_{10} = q\cO_{10} + 3q\cO'_{10} - 3q\cO'_{11}$;\\
$\cO_{12} \star \cO'_{10} = q\cO_{10} + q\cO'_{10} - q\cO'_{11}$ ;
$\cO_{12} \star \cO_{11} = 2q\cO'_{11} - q\cO_{12}$ ;\\
$\cO_{12} \star \cO'_{11} = q\cO_{11} + 2q\cO'_{11} - q\cO_{12} - 2q\cO'_{12} + q\cO_{13}$ ;
$\cO_{12} \star \cO_{12} = q\cO_{12} + q\cO'_{12} + q^2 - q\cO_{13} - q^2\cO_{1}$ ;\\
$\cO'_{12} \star \cO_{1} = \cO_{13} + q\cO_{1} - q\cO_{2}$ ;
$\cO'_{12} \star \cO_{2} = \cO_{14} + 2q\cO_{2} - 2q\cO_{3}$ ;\\
$\cO'_{12} \star \cO_{3} = \cO_{15} + 3q\cO_{3} - 2q\cO_{4} - 3q\cO'_{4} + 2q\cO'_{5}$ ;
$\cO'_{12} \star \cO_{4} = q\cO_{4} + 2q\cO'_{4} - 2q\cO'_{5}$ ;\\
$\cO'_{12} \star \cO'_{4} = \cO_{16} + 2q\cO_{4} + 2q\cO'_{4} - 2q\cO_{5} - 3q\cO'_{5} + q\cO_{6}$ ;
$\cO'_{12} \star \cO_{5} = q\cO_{5} + q\cO'_{5} - q\cO_{6}$ ;\\
$\cO'_{12} \star \cO'_{5} = 2q\cO_{5} + 3q\cO'_{5} - 4q\cO_{6} - 2q\cO'_{6} + 2q\cO_{7}$ ;
$\cO'_{12} \star \cO_{6} = 2q\cO_{6} + q\cO'_{6} - 2q\cO_{7}$ ;\\
$\cO'_{12} \star \cO'_{6} = 3q\cO_{6} + 2q\cO'_{6} - 4q\cO_{7} - q\cO'_{7} + q\cO'_{8}$ ;
$\cO'_{12} \star \cO_{7} = 3q\cO_{7} + q\cO'_{7} - 2q\cO_{8} - 3q\cO'_{8} + 2q\cO_{9}$ ;\\
$\cO'_{12} \star \cO'_{7} = 2q\cO_{7} + q\cO'_{7} - 2q\cO'_{8}$ ;
$\cO'_{12} \star \cO_{8} = q\cO_{8} + 2q\cO'_{8} - 2q\cO_{9}$ ;\\
$\cO'_{12} \star \cO'_{8} = 2q\cO_{8} + 2q\cO'_{8} + q\cO''_{8} - 3q\cO_{9} - 2q\cO'_{9} + q\cO'_{10}$ ;
$\cO'_{12} \star \cO''_{8} = q\cO'_{8}$ ;\\
$\cO'_{12} \star \cO_{9} = 3q\cO_{9} + 2q\cO'_{9} - 2q\cO_{10} - 4q\cO'_{10} + 2q\cO'_{11}$ ;
$\cO'_{12} \star \cO'_{9} = q\cO_{9} + q\cO'_{9} - q\cO'_{10}$ ;\\
$\cO'_{12} \star \cO_{10} = 2q\cO_{10} + 3q\cO'_{10} - q\cO_{11} - 4q\cO'_{11} + q\cO'_{12}$ ;
$\cO'_{12} \star \cO'_{10} = q\cO_{10} + 2q\cO'_{10} - 2q\cO'_{11}$ ;\\
$\cO'_{12} \star \cO_{11} = q\cO_{11} + 2q\cO'_{11} - 2q\cO'_{12}$ ;
$\cO'_{12} \star \cO'_{11} = q\cO_{11} + 3q\cO'_{11} - 2q\cO_{12} - 3q\cO'_{12} + 2q\cO_{13}$ ;\\
$\cO'_{12} \star \cO_{12} = q\cO_{12} + 2q\cO'_{12} - 2q\cO_{13}$ ;
$\cO'_{12} \star \cO'_{12} = 2q\cO_{12} + 2q\cO'_{12} + q^2 - 3q\cO_{13} - 2q^2\cO_{1} + q^2\cO_{2}$ ;\\
$\cO_{13} \star \cO_{1} = \cO_{14} + q\cO_{2} - q\cO_{3}$ ;
$\cO_{13} \star \cO_{2} = \cO_{15} + 2q\cO_{3} - q\cO_{4} - 2q\cO'_{4} + q\cO'_{5}$ ;\\
$\cO_{13} \star \cO_{3} = \cO_{16} + 2q\cO_{4} + 3q\cO'_{4} - 3q\cO_{5} - 5q\cO'_{5} + 3q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;\\
$\cO_{13} \star \cO_{4} = 2q\cO_{5} + 2q\cO'_{5} - 3q\cO_{6} - q\cO'_{6} + q\cO_{7}$ ;
$\cO_{13} \star \cO'_{4} = 2q\cO_{5} + 3q\cO'_{5} - 4q\cO_{6} - 2q\cO'_{6} + 2q\cO_{7}$ ;\\
$\cO_{13} \star \cO_{5} = q\cO_{6} + q\cO'_{6} - q\cO_{7}$ ;
$\cO_{13} \star \cO'_{5} = 4q\cO_{6} + 2q\cO'_{6} - 6q\cO_{7} - q\cO'_{7} + q\cO_{8} + 2q\cO'_{8} - q\cO_{9}$ ;\\
$\cO_{13} \star \cO_{6} = 2q\cO_{7} + q\cO'_{7} - q\cO_{8} - 2q\cO'_{8} + q\cO_{9}$ ;
$\cO_{13} \star \cO'_{6} = 4q\cO_{7} + q\cO'_{7} - 3q\cO_{8} - 4q\cO'_{8} + 3q\cO_{9}$ ;\\
$\cO_{13} \star \cO_{7} = 2q\cO_{8} + 3q\cO'_{8} + q\cO''_{8} - 5q\cO_{9} - 3q\cO'_{9} + q\cO_{10} + 3q\cO'_{10} - q\cO'_{11}$ ;\\
$\cO_{13} \star \cO'_{7} = 2q\cO_{8} + 2q\cO'_{8} - 3q\cO_{9}$ ;
$\cO_{13} \star \cO_{8} = 2q\cO_{9} + 2q\cO'_{9} - q\cO_{10} - 3q\cO'_{10} + q\cO'_{11}$ ;\\
$\cO_{13} \star \cO'_{8} = 3q\cO_{9} + 2q\cO'_{9} - 2q\cO_{10} - 4q\cO'_{10} + 2q\cO'_{11}$ ;
$\cO_{13} \star \cO''_{8} = q\cO_{9}$ ;\\
$\cO_{13} \star \cO_{9} = 2q\cO_{10} + 4q\cO'_{10} - q\cO_{11} - 6q\cO'_{11} + q\cO_{12} + 2q\cO'_{12} - q\cO_{13}$ ;
$\cO_{13} \star \cO'_{9} = q\cO_{10} + q\cO'_{10} - q\cO'_{11}$ ;\\
$\cO_{13} \star \cO_{10} = q\cO_{11} + 4q\cO'_{11} - 3q\cO_{12} - 4q\cO'_{12} + 3q\cO_{13}$ ;
$\cO_{13} \star \cO'_{10} = q\cO_{11} + 2q\cO'_{11} - q\cO_{12} - 2q\cO'_{12} + q\cO_{13}$;\\
$\cO_{13} \star \cO_{11} = 2q\cO_{12} + 2q\cO'_{12} - 3q\cO_{13}$ ;\\
$\cO_{13} \star \cO'_{11} = 2q\cO_{12} + 3q\cO'_{12} + q^2 - 5q\cO_{13} - 3q^2\cO_{1} + q\cO_{14} + 3q^2\cO_{2} - q^2\cO_{3}$ ;\\
$\cO_{13} \star \cO_{12} = 2q\cO_{13} + 2q^2\cO_{1} - q\cO_{14} - 3q^2\cO_{2} + q^2\cO_{3}$ ;\\
$\cO_{13} \star \cO'_{12} = 3q\cO_{13} + 2q^2\cO_{1} - 2q\cO_{14} - 4q^2\cO_{2} + 2q^2\cO_{3}$ ;\\
$\cO_{13} \star \cO_{13} = 2q\cO_{14} + 4q^2\cO_{2} - q\cO_{15} - 6q^2\cO_{3} + q^2\cO_{4} + 2q^2\cO'_{4} - q^2\cO'_{5}$ ;\\
$\cO_{14} \star \cO_{1} = \cO_{15} + q\cO_{3} - q\cO'_{4}$ ;
$\cO_{14} \star \cO_{2} = \cO_{16} + q\cO_{4} + 2q\cO'_{4} - 2q\cO_{5} - 2q\cO'_{5} + q\cO_{6}$ ;\\
$\cO_{14} \star \cO_{3} = 3q\cO_{5} + 3q\cO'_{5} - 6q\cO_{6} - 2q\cO'_{6} + 3q\cO_{7}$ ;
$\cO_{14} \star \cO_{4} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$ ;\\
$\cO_{14} \star \cO'_{4} = 3q\cO_{6} + 2q\cO'_{6} - 4q\cO_{7} - q\cO'_{7} + q\cO'_{8}$ ;
$\cO_{14} \star \cO_{5} = q\cO_{7} + q\cO'_{7} - q\cO'_{8}$ ;\\
$\cO_{14} \star \cO'_{5} = 4q\cO_{7} + q\cO'_{7} - 3q\cO_{8} - 4q\cO'_{8} + 3q\cO_{9}$ ;
$\cO_{14} \star \cO_{6} = q\cO_{8} + 2q\cO'_{8} + q\cO''_{8} - 2q\cO_{9} - 2q\cO'_{9} + q\cO'_{10}$ ;\\
$\cO_{14} \star \cO'_{6} = 3q\cO_{8} + 3q\cO'_{8} - 6q\cO_{9} + q\cO_{10}$ ;
$\cO_{14} \star \cO_{7} = 3q\cO_{9} + 3q\cO'_{9} - 2q\cO_{10} - 6q\cO'_{10} + 3q\cO'_{11}$ ;\\
$\cO_{14} \star \cO'_{7} = 3q\cO_{9} - 2q\cO_{10}$ ;
$\cO_{14} \star \cO_{8} = q\cO_{10} + 3q\cO'_{10} - 3q\cO'_{11}$ ;\\
$\cO_{14} \star \cO'_{8} = 2q\cO_{10} + 3q\cO'_{10} - q\cO_{11} - 4q\cO'_{11} + q\cO'_{12}$ ;
$\cO_{14} \star \cO''_{8} = q\cO_{10}$ ;\\
$\cO_{14} \star \cO_{9} = q\cO_{11} + 4q\cO'_{11} - 3q\cO_{12} - 4q\cO'_{12} + 3q\cO_{13}$ ;
$\cO_{14} \star \cO'_{9} = q\cO_{11} + q\cO'_{11} - q\cO'_{12}$ ;\\
$\cO_{14} \star \cO_{10} = 3q\cO_{12} + 3q\cO'_{12} - 6q\cO_{13} + q\cO_{14}$ ;
$\cO_{14} \star \cO'_{10} = q\cO_{12} + 2q\cO'_{12} + q^2 - 2q\cO_{13} - 2q^2\cO_{1} + q^2\cO_{2}$ ;\\
$\cO_{14} \star \cO_{11} = 3q\cO_{13} - 2q\cO_{14}$ ;
$\cO_{14} \star \cO'_{11} = 3q\cO_{13} + 3q^2\cO_{1} - 2q\cO_{14} - 6q^2\cO_{2} + 3q^2\cO_{3}$ ;\\
$\cO_{14} \star \cO_{12} = q\cO_{14} + 3q^2\cO_{2} - 3q^2\cO_{3}$ ;
$\cO_{14} \star \cO'_{12} = 2q\cO_{14} + 3q^2\cO_{2} - q\cO_{15} - 4q^2\cO_{3} + q^2\cO'_{4}$ ;\\
$\cO_{14} \star \cO_{13} = q\cO_{15} + 4q^2\cO_{3} - 3q^2\cO_{4} - 4q^2\cO'_{4} + 3q^2\cO'_{5}$ ;
$\cO_{14} \star \cO_{14} = 3q^2\cO_{4} + 3q^2\cO'_{4} - 6q^2\cO'_{5} + q^2\cO'_{6}$ ;\\
$\cO_{15} \star \cO_{1} = \cO_{16} + q\cO'_{4} - q\cO_{5}$ ;
$\cO_{15} \star \cO_{2} = 2q\cO_{5} + q\cO'_{5} - 2q\cO_{6}$ ;
$\cO_{15} \star \cO_{3} = 3q\cO_{6} + q\cO'_{6} - 3q\cO_{7}$ ;\\
$\cO_{15} \star \cO_{4} = 2q\cO_{7} - q\cO_{8}$ ;
$\cO_{15} \star \cO'_{4} = 2q\cO_{7} + q\cO'_{7} - 2q\cO'_{8}$ ;
$\cO_{15} \star \cO_{5} = q\cO'_{8} + q\cO''_{8} - q\cO'_{9}$ ;\\
$\cO_{15} \star \cO'_{5} = 2q\cO_{8} + 2q\cO'_{8} - 3q\cO_{9}$ ;
$\cO_{15} \star \cO_{6} = q\cO_{9} + 2q\cO'_{9} - 2q\cO'_{10}$ ;
$\cO_{15} \star \cO'_{6} = 3q\cO_{9} - 2q\cO_{10}$ ;\\
$\cO_{15} \star \cO_{7} = q\cO_{10} + 3q\cO'_{10} - 3q\cO'_{11}$ ;
$\cO_{15} \star \cO'_{7} = 2q\cO_{10} - q\cO_{11}$ ;
$\cO_{15} \star \cO_{8} = 2q\cO'_{11} - q\cO_{12}$ ;\\
$\cO_{15} \star \cO'_{8} = q\cO_{11} + 2q\cO'_{11} - 2q\cO'_{12}$ ;
$\cO_{15} \star \cO''_{8} = q\cO_{11}$ ;
$\cO_{15} \star \cO_{9} = 2q\cO_{12} + 2q\cO'_{12} - 3q\cO_{13}$ ;\\
$\cO_{15} \star \cO'_{9} = q\cO'_{12} + q^2 - q^2\cO_{1}$ ;
$\cO_{15} \star \cO_{10} = 3q\cO_{13} - 2q\cO_{14}$ ;
$\cO_{15} \star \cO'_{10} = q\cO_{13} + 2q^2\cO_{1} - 2q^2\cO_{2}$ ;\\
$\cO_{15} \star \cO_{11} = 2q\cO_{14} - q\cO_{15}$ ;
$\cO_{15} \star \cO'_{11} = q\cO_{14} + 3q^2\cO_{2} - 3q^2\cO_{3}$ ;
$\cO_{15} \star \cO_{12} = 2q^2\cO_{3} - q^2\cO_{4}$ ;\\
$\cO_{15} \star \cO'_{12} = q\cO_{15} + 2q^2\cO_{3} - 2q^2\cO'_{4}$ ;
$\cO_{15} \star \cO_{13} = 2q^2\cO_{4} + 2q^2\cO'_{4} - 3q^2\cO'_{5}$ ;
$\cO_{15} \star \cO_{14} = 3q^2\cO'_{5} - 2q^2\cO'_{6}$;\\
$\cO_{15} \star \cO_{15} = 2q^2\cO'_{6} - q^2\cO'_{7}$ ;
$\cO_{16} \star \cO_{1} = q\cO_{5}$ ;
$\cO_{16} \star \cO_{2} = q\cO_{6}$ ;
$\cO_{16} \star \cO_{3} = q\cO_{7}$ ;
$\cO_{16} \star \cO_{4} = q\cO_{8}$ ;\\
$\cO_{16} \star \cO'_{4} = q\cO'_{8}$ ;
$\cO_{16} \star \cO_{5} = q\cO'_{9}$ ;
$\cO_{16} \star \cO'_{5} = q\cO_{9}$ ;
$\cO_{16} \star \cO_{6} = q\cO'_{10}$ ;
$\cO_{16} \star \cO'_{6} = q\cO_{10}$ ;\\
$\cO_{16} \star \cO_{7} = q\cO'_{11}$ ;
$\cO_{16} \star \cO'_{7} = q\cO_{11}$ ;
$\cO_{16} \star \cO_{8} = q\cO_{12}$ ;
$\cO_{16} \star \cO'_{8} = q\cO'_{12}$ ;
$\cO_{16} \star \cO''_{8} = q^2$ ;\\
$\cO_{16} \star \cO_{9} = q\cO_{13}$ ;
$\cO_{16} \star \cO'_{9} = q^2\cO_{1}$ ;
$\cO_{16} \star \cO_{10} = q\cO_{14}$ ;
$\cO_{16} \star \cO'_{10} = q^2\cO_{2}$ ;
$\cO_{16} \star \cO_{11} = q\cO_{15}$ ;\\
$\cO_{16} \star \cO'_{11} = q^2\cO_{3}$ ;
$\cO_{16} \star \cO_{12} = q^2\cO_{4}$ ;
$\cO_{16} \star \cO'_{12} = q^2\cO'_{4}$ ;
$\cO_{16} \star \cO_{13} = q^2\cO'_{5}$ ;
$\cO_{16} \star \cO_{14} = q^2\cO'_{6}$ ;\\
$\cO_{16} \star \cO_{15} = q^2\cO'_{7}$ ;
$\cO_{16} \star \cO_{16} = q^2\cO''_{8}$
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "qkfinite"
%%% End: 

% LocalWords:  RHS FW Comin FIXME

